SparseAdapter: An Easy Approach for Improving the Parameter-Efficiency of Adapters

Adapter Tuning, which freezes the pretrained language models (PLMs) and only fine-tunes a few extra modules, becomes an appealing efficient alternative to the full model fine-tuning. Although computationally efficient, the recent Adapters often increase parameters (e.g. bottleneck dimension) for matching the performance of full model fine-tuning, which we argue goes against their original intention. In this work, we re-examine the parameter-efficiency of Adapters through the lens of network pruning (we name such plug-in concept as \texttt{SparseAdapter}) and find that SparseAdapter can achieve comparable or better performance than standard Adapters when the sparse ratio reaches up to 80\%. Based on our findings, we introduce an easy but effective setting ``\textit{Large-Sparse}'' to improve the model capacity of Adapters under the same parameter budget. Experiments on five competitive Adapters upon three advanced PLMs show that with proper sparse method (e.g. SNIP) and ratio (e.g. 40\%) SparseAdapter can consistently outperform their corresponding counterpart. Encouragingly, with the \textit{Large-Sparse} setting, we can obtain further appealing gains, even outperforming the full fine-tuning by a large margin. Our code will be released at: https://github.com/Shwai-He/SparseAdapter.

==> RelatedWork.tex <==
\section{RelatedWork}
\label{:sec:RelatedWork}
\textbf{Adapter}
Adapter layers (or adapters for short) were first
proposed in computer vision \cite{rebuffi2017learning},
then extended for text classification tasks in
NLP \cite{houlsby2019parameter}. Till now, adapters have been explored in many other natural language task, including neural machine translation \cite{bapna-firat-2019-simple}, multi-task cross-lingual transfer \cite{pfeiffer-etal-2020-mad}. Adapters are generally inserted between the layers of a pre-trained network
and finetuned on the adaptation corpus. There also emerge many variants for adapters. Pfeiffer \cite{pfeiffer2020adapterfusion} proposes AdapterFusion to combine various types of knowledge at different layers of the model. Hu \cite{hu2021lora}~\textit{et al.} propose LORA that injects trainable rank-decomposition matrices into each layer of the Transformer architecture, greatly reducing the number of trainable parameters for downstream tasks. 

\textbf{Pruning At Initialization}
Pruning \cite{lecun1989optimal} aims to remove unimportant
weights from a neural network to achieve parameter-efficiency
while preserving model performance. According to the time point to prune, existing pruning works can be categorized into three groups \cite{liu2021sparse}:  Post-Training Pruning \cite{han2015learning, molchanov2016pruning, lin2020dynamic}, During-Training Pruning \cite{mocanu2018scalable, evci2020rigging}, and Before-Training Pruning \cite{lee2018snip,  tanaka2020pruning, wang2020picking}. During-Training Pruning and Post-Training Pruning often require iterative operations: training, pruning, and retraining. Instead of pruning iteratively, Before-Training Pruning attempts to find a sub-structure before training and train the rest parameters once, reducing the computational cost to find the pruned structure. Many works \cite{wang2020picking, lee2018snip, tanaka2020pruning} have explored the possibility of obtaining a trainable sparse neural network before the main training process. \cite{frankle2020pruning} demonstrates that the existing methods for pruning at initialization can perform equally with the dense model. 

